Coalitional Bayesian Autoencoders -- Towards explainable unsupervised deep learning

This paper aims to improve the explainability of Autoencoder's (AE) predictions by proposing two explanation methods based on the mean and epistemic uncertainty of log-likelihood estimate, which naturally arise from the probabilistic formulation of the AE called Bayesian Autoencoders (BAE). To quantitatively evaluate the performance of explanation methods, we test them in sensor network applications, and propose three metrics based on covariate shift of sensors : (1) G-mean of Spearman drift coefficients, (2) G-mean of sensitivity-specificity of explanation ranking and (3) sensor explanation quality index (SEQI) which combines the two aforementioned metrics. Surprisingly, we find that explanations of BAE's predictions suffer from high correlation resulting in misleading explanations. To alleviate this, a "Coalitional BAE" is proposed, which is inspired by agent-based system theory. Our comprehensive experiments on publicly available condition monitoring datasets demonstrate the improved quality of explanations using the Coalitional BAE.

==> tables/model_architecture.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\caption{Encoder architecture of BAE for PRONOSTIA and ZEMA datasets. The decoder is a reflection of the encoder without the dense latent layer, and the convolution layers are replaced by convolution transpose layers.}
\label{table-architecture}
\centering
% \vskip 0.1in
\begin{tabular}{@{}cccc@{}}
\toprule
Layer       & Output channels/nodes & Kernel size & Strides \\ \midrule
1D-Convolution & 8      & 20  & 4   \\
1D-Convolution & 5      & 10  & 2   \\
Flatten     & -              & -      & -       \\
Dense       & 150       & -      & -      \\
Dense (latent)      & 20       & -      & -      \\ \bottomrule

\end{tabular}
\end{table}
% \newline \newline
% b) CIFAR10 and SVHN
% \begin{tabular}{@{}cccc@{}}
% \toprule
% Layer       & Output dimensions & Kernel & Strides \\ \midrule
% Convolution & 15 x 15 x 32      & 4 x 4  & 2 x 2   \\
% Convolution & 12 x 12 x 64      & 4 x 4  & 1 x 1   \\
% Convolution & 5 x 5 x 128       & 4 x 4  & 2 x 2   \\
% Reshape     & 3200              & -      & -       \\
% Dense       & Latent size       & -      & -      \\ \bottomrule
% \end{tabular}
% \end{table}

==> tables/prognostia_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}llllll@{}}
\toprule
bae\_type & coalition & mu\_var        & SPMAN & GMEAN & TOTAL\_NLL \\ \midrule
ae        & central   & mu             & 0.606 & 0.842 & 0.724      \\ \cmidrule(l){3-6} 
          &           & deeplift       & 0.478 & 0.623 & 0.55       \\ \cmidrule(l){3-6} 
          &           & gradient\_shap & 0.588 & 0.38  & 0.484      \\ \cmidrule(l){2-6} 
          & coalition & mu             & 0.701 & 0.865 & 0.783      \\ \midrule
bae       & central   & mu             & 0.61  & 0.843 & 0.726      \\ \cmidrule(l){3-6} 
          &           & var            & 0.574 & 0.99  & 0.782      \\ \cmidrule(l){2-6} 
          & coalition & mu             & 0.704 & 0.865 & 0.784      \\ \cmidrule(l){3-6} 
          &           & var            & 0.77  & 0.961 & 0.865      \\ \bottomrule
\end{tabular}
\end{table}

==> tables/pronostia_gmean_sdc_maxrow.tex <==
%Table - PRONOSTIA GMEAN SDC
\begin{table}[!ht]
\centering
\caption{Mean and standard error of $G_{SDC}$ (0 = worst score, 1 = perfect score) for various explanation methods with varied number of convolution layers and model capacities evaluated on (a) PRONOSTIA and (b) ZEMA datasets. Highest mean value of each column is bolded. * indicates overall highest value. }
\scriptsize  (a) PRONOSTIA

\label{table-results-zema}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllll}
\hline
&  &  & \multicolumn{9}{c}{G-mean of Spearman drift coefficients ($G_{SDC}$)} \\ \cline{4-12} 
&  &  & \multicolumn{3}{c}{1 Convolution Layer} & \multicolumn{3}{c}{2 Convolution Layers} & \multicolumn{3}{c}{3 Convolution Layers}  \\ \cline{4-12} 

    % &           &          & \multicolumn{3}{c|}{Capacity x$\frac{1}{2}$}                                                                      & \multicolumn{3}{c|}{Capacity x$1$}                                                                     & \multicolumn{3}{c}{Capacity x$2$}                                                                                 \\ \cline{4-12} 
    
% \multicolumn{3}{c}{Method \textbackslash{ Capacity }} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} &

% \multicolumn{3}{c}{\backslashbox{Room}{Date}} &
% \multicolumn{1}{c}{x$\frac{1}{4}$} & \multicolumn{1}{c}{x$1$} &

\multicolumn{3}{c}{Method \textbackslash{ Capacity }} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} &
\multicolumn{1}{c}{x$2$} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} & \multicolumn{1}{c}{x$2$} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} & \multicolumn{1}{c}{x$2$} \\ \hline

% \multicolumn{3}{c}{Method \textbackslash{ Layers }} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} &
% \multicolumn{1}{c|}{3}
% & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c|}{3} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} \\ \hline

AE  & Central   & \exLL{} &    
0.606$\pm{}$0.038&0.566$\pm{}$0.035&0.584$\pm{}$0.039&0.594$\pm{}$0.038&0.547$\pm{}$0.041&0.552$\pm{}$0.037&\textBF{0.653$\pm{}$0.036}&0.633$\pm{}$0.039&0.573$\pm{}$0.043

\\ \cline{3-12}  &           & DeepLIFT & 
0.500$\pm{}$0.042&0.419$\pm{}$0.035&0.396$\pm{}$0.040&0.487$\pm{}$0.048&0.366$\pm{}$0.044&0.407$\pm{}$0.040&\textBF{0.537$\pm{}$0.043}&0.452$\pm{}$0.035&0.386$\pm{}$0.040

\\ \cline{3-12}  &           & GradShap & 
\textBF{0.558$\pm{}$0.030}&0.522$\pm{}$0.034&0.531$\pm{}$0.030&0.529$\pm{}$0.031&0.511$\pm{}$0.023&0.481$\pm{}$0.030&0.530$\pm{}$0.026&0.489$\pm{}$0.028&0.487$\pm{}$0.032

\\ \cline{2-12}  & Coalition & \exLL{}     & 
0.714$\pm{}$0.037&\textBF{*0.742$\pm{}$0.031}&0.715$\pm{}$0.028&0.668$\pm{}$0.034&0.694$\pm{}$0.031&0.698$\pm{}$0.033&0.682$\pm{}$0.032&0.661$\pm{}$0.043&0.707$\pm{}$0.030


\\ \hline BAE & Central   & \exLL{}     &
0.527$\pm{}$0.037&0.527$\pm{}$0.032&0.557$\pm{}$0.037&0.574$\pm{}$0.037&0.560$\pm{}$0.041&0.525$\pm{}$0.036&\textBF{0.676$\pm{}$0.035}&0.598$\pm{}$0.041&0.603$\pm{}$0.038
 
\\ \cline{3-12}   &           & \varLL{}    &
0.456$\pm{}$0.037&0.449$\pm{}$0.033&0.467$\pm{}$0.038&0.370$\pm{}$0.040&0.425$\pm{}$0.045&0.336$\pm{}$0.044&\textBF{0.701$\pm{}$0.040}&0.404$\pm{}$0.041&0.358$\pm{}$0.044

\\ \cline{2-12}  & Coalition & \exLL{}     & 
0.682$\pm{}$0.038&0.716$\pm{}$0.029&\textBF{0.719$\pm{}$0.030}&0.638$\pm{}$0.041&0.660$\pm{}$0.038&0.680$\pm{}$0.039&0.673$\pm{}$0.033&0.691$\pm{}$0.033&0.696$\pm{}$0.032

\\ \cline{3-12}  &  & \varLL{}   &
0.649$\pm{}$0.041&0.630$\pm{}$0.036&0.613$\pm{}$0.035&0.712$\pm{}$0.034&0.696$\pm{}$0.032&0.655$\pm{}$0.037&0.705$\pm{}$0.036&\textBF{0.726$\pm{}$0.034}&0.685$\pm{}$0.033


    \\ \hline
\end{tabular}
}
\end{table}

==> tables/zema_gmean_sdc_maxrow.tex <==
%Table - PRONOSTIA GMEAN SDC
\begin{table}[!ht]
\centering
\scriptsize  (b) ZEMA
\label{table-results-zema}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllll}
\hline
&  &  & \multicolumn{9}{c}{G-mean of Spearman drift coefficients ($G_{SDC}$)} \\ \cline{4-12} 
&  &  & \multicolumn{3}{c}{1 Convolution Layer} & \multicolumn{3}{c}{2 Convolution Layers} & \multicolumn{3}{c}{3 Convolution Layers}  \\ \cline{4-12} 
    % &           &          & \multicolumn{3}{c|}{Capacity x$\frac{1}{2}$}                                                                      & \multicolumn{3}{c|}{Capacity x$1$}                                                                     & \multicolumn{3}{c}{Capacity x$2$}                                                                                 \\ \cline{4-12} 
    
% \multicolumn{3}{c}{Method \textbackslash{ Capacity }} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} &

% \multicolumn{3}{c}{\backslashbox{Room}{Date}} &
% \multicolumn{1}{c}{x$\frac{1}{4}$} & \multicolumn{1}{c}{x$1$} &

\multicolumn{3}{c}{Method \textbackslash{ Capacity }} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} &
\multicolumn{1}{c}{x$2$} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} & \multicolumn{1}{c}{x$2$} & \multicolumn{1}{c}{x$\frac{1}{2}$} & \multicolumn{1}{c}{x$1$} & \multicolumn{1}{c}{x$2$} \\ \hline

% \multicolumn{3}{c}{Method \textbackslash{ Layers }} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} &
% \multicolumn{1}{c|}{3}
% & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c|}{3} & \multicolumn{1}{c}{1} & \multicolumn{1}{c}{2} & \multicolumn{1}{c}{3} \\ \hline

AE  & Central   & \exLL{} &    
\textBF{0.643$\pm{}$0.023}&0.620$\pm{}$0.023&0.595$\pm{}$0.025&0.604$\pm{}$0.025&0.619$\pm{}$0.026&0.574$\pm{}$0.025&0.624$\pm{}$0.024&0.587$\pm{}$0.025&0.583$\pm{}$0.024

\\ \cline{3-12}  &           & DeepLIFT & 
0.436$\pm{}$0.022&0.454$\pm{}$0.025&0.436$\pm{}$0.026&0.478$\pm{}$0.022&0.462$\pm{}$0.025&0.442$\pm{}$0.025&\textBF{0.562$\pm{}$0.029}&0.474$\pm{}$0.025&0.501$\pm{}$0.024

\\ \cline{3-12}  &           & GradShap & 
0.490$\pm{}$0.020&0.458$\pm{}$0.021&0.454$\pm{}$0.023&0.540$\pm{}$0.022&0.570$\pm{}$0.022&0.486$\pm{}$0.025&\textBF{0.578$\pm{}$0.026}&0.526$\pm{}$0.022&0.567$\pm{}$0.024

\\ \cline{2-12}  & Coalition & \exLL{}     & 
0.648$\pm{}$0.024&0.659$\pm{}$0.025&\textBF{0.672$\pm{}$0.024}&0.659$\pm{}$0.021&0.647$\pm{}$0.025&0.640$\pm{}$0.024&0.654$\pm{}$0.021&0.646$\pm{}$0.022&0.627$\pm{}$0.027


\\ \hline BAE & Central   & \exLL{}     &
0.638$\pm{}$0.023&0.604$\pm{}$0.025&0.578$\pm{}$0.026&0.615$\pm{}$0.024&0.597$\pm{}$0.025&0.548$\pm{}$0.026&\textBF{0.644$\pm{}$0.024}&0.592$\pm{}$0.024&0.600$\pm{}$0.024

\\ \cline{3-12}   &           & \varLL{}    &
0.560$\pm{}$0.022&0.498$\pm{}$0.020&0.473$\pm{}$0.019&0.533$\pm{}$0.017&0.505$\pm{}$0.021&0.493$\pm{}$0.021&\textBF{0.566$\pm{}$0.018}&0.516$\pm{}$0.015&0.528$\pm{}$0.020

\\ \cline{2-12}  & Coalition & \exLL{}     & 
0.659$\pm{}$0.024&\textBF{0.675$\pm{}$0.026}&0.675$\pm{}$0.024&0.653$\pm{}$0.023&0.648$\pm{}$0.024&0.647$\pm{}$0.023&0.643$\pm{}$0.023&0.648$\pm{}$0.023&0.632$\pm{}$0.023


\\ \cline{3-12}  &  & \varLL{}   &
\textBF{*0.680$\pm{}$0.019}&0.621$\pm{}$0.020&0.650$\pm{}$0.020&0.645$\pm{}$0.019&0.660$\pm{}$0.019&0.620$\pm{}$0.021&0.595$\pm{}$0.019&0.631$\pm{}$0.020&0.631$\pm{}$0.020


    \\ \hline
\end{tabular}
}
\end{table}

==> tables/zema_table.tex <==
%Table 1 - FashionMNIST vs MNIST
\begin{table}[!ht]
\centering
\caption{(FashionMNIST vs MNIST) AUROC for detecting OOD inputs with deterministic AE, VAE and BAE (MC-Dropout, Bayes by Backprop and anchored ensembling) with posterior approximated under various techniques. For each likelihood- Bernoulli, Continuous Bernoulli and Gaussian, we compare the performance of using $\mathrm{Var}_\theta(\hat{\textBF{x}})$, $\E_{\theta}\mathrm{(LL)}$, $\mathrm{Var_{\theta}(LL)}$, and WAIC. Top 2 results for each model capacity are bolded.}
\label{table-results-zema}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllllll}
\hline
    &           &          & \multicolumn{3}{c}{SPMAN}                                                                      & \multicolumn{3}{c}{G MEAN}                                                                     & \multicolumn{3}{c}{TOTAL NLL}                                                                                 \\ \cline{4-12} 
\multicolumn{3}{c}{Method} & \multicolumn{1}{c}{x$\frac{1}{4}$} & \multicolumn{1}{c}{x$1$} & \multicolumn{1}{c}{x$4$} & \multicolumn{1}{c}{x$\frac{1}{4}$} & \multicolumn{1}{c}{x$1$} & \multicolumn{1}{c}{x$4$} & \multicolumn{1}{c}{x$\frac{1}{4}$} & \multicolumn{1}{c}{x$1$} & \multicolumn{1}{c}{x$4$} \\ \hline
AE  & Central   & \exLL{}     & 0.707$\pm{}$0.007                   & 0.657$\pm{}$0.008                  & 0.653$\pm{}$0.008                  & 0.603$\pm{}$0.019                   & 0.615$\pm{}$0.019                  & 0.647$\pm{}$0.018                  & 0.655$\pm{}$0.011                        & 0.636$\pm{}$0.011                       & 0.650$\pm{}$0.011                        \\ \cline{3-12} 
    &           & DeepLIFT & 0.630$\pm{}$0.01                     & 0.465$\pm{}$0.009                  & 0.437$\pm{}$0.008                  & 0.547$\pm{}$0.022                   & 0.527$\pm{}$0.021                  & 0.534$\pm{}$0.020                   & 0.588$\pm{}$0.013                        & 0.496$\pm{}$0.013                       & 0.485$\pm{}$0.012                       \\ \cline{3-12} 
    &           & GradShap & 0.628$\pm{}$0.009                   & 0.494$\pm{}$0.008                  & 0.488$\pm{}$0.007                  & 0.164$\pm{}$0.013                   & 0.228$\pm{}$0.015                  & 0.248$\pm{}$0.016                  & 0.396$\pm{}$0.007                        & 0.361$\pm{}$0.009                       & 0.368$\pm{}$0.009                       \\ \cline{2-12} 
    & Coalition & \exLL{}     & \textBF{0.720$\pm{}$0.007}              & \textBF{0.699$\pm{}$0.009}            & \textBF{0.698$\pm{}$0.009}            & 0.607$\pm{}$0.020                    & 0.605$\pm{}$0.020                   & 0.596$\pm{}$0.020                   & 0.664$\pm{}$0.011                        & 0.652$\pm{}$0.011                       & 0.647$\pm{}$0.012                       \\ \hline
BAE & Central   & \exLL{}     & 0.702$\pm{}$0.008                   & 0.644$\pm{}$0.008                  & 0.641$\pm{}$0.008                  & 0.628$\pm{}$0.019                   & 0.642$\pm{}$0.018                  & 0.630$\pm{}$0.019                   & 0.665$\pm{}$0.011                        & 0.643$\pm{}$0.010                        & 0.635$\pm{}$0.011                       \\ \cline{3-12} 
    &           & \varLL{}    & 0.620$\pm{}$0.009                    & 0.548$\pm{}$0.010                   & 0.578$\pm{}$0.010                   & \textBF{0.848$\pm{}$0.015}             & \textBF{0.924$\pm{}$0.008}            & \textBF{0.936$\pm{}$0.007}            & \textBF{0.734$\pm{}$0.009}                  & \textBF{0.736$\pm{}$0.006}                 & \textBF{0.757$\pm{}$0.006}                \\ \cline{2-12} 
    & Coalition & \exLL{}     & \textBF{0.720$\pm{}$0.007}              & 0.693$\pm{}$0.009                  & \textBF{0.698$\pm{}$0.009}            & 0.602$\pm{}$0.020                    & 0.606$\pm{}$0.020                   & 0.619$\pm{}$0.019                  & 0.661$\pm{}$0.011                        & 0.650$\pm{}$0.011                        & 0.658$\pm{}$0.011                       \\ \cline{3-12} 
    &           & \varLL{}    & 0.713$\pm{}$0.008                   & \textBF{0.752$\pm{}$0.007}            & \textBF{0.722$\pm{}$0.008}            & \textBF{0.803$\pm{}$0.016}             & \textBF{0.895$\pm{}$0.015}            & \textBF{0.832$\pm{}$0.018}            & \textBF{0.758$\pm{}$0.009}                  & \textBF{0.824$\pm{}$0.008}                 & \textBF{0.777$\pm{}$0.009}                 \\ \hline
\end{tabular}
}
\end{table}

==> tables/zema_table_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}llllllllllll@{}}
\toprule
    &           &                           & \multicolumn{3}{c}{SPMAN}                                                                          & \multicolumn{3}{c}{G MEAN}                                                                          & \multicolumn{3}{c}{TOTAL NLL}                                                                                 \\ \cmidrule(l){4-12} 
\multicolumn{3}{c}{Method}                  & \multicolumn{1}{c}{SPMAN-0.25} & \multicolumn{1}{c}{SPMAN-1.0}   & \multicolumn{1}{c}{SPMAN-4.0}   & \multicolumn{1}{c}{GMEAN-0.25}  & \multicolumn{1}{c}{GMEAN-1.0}   & \multicolumn{1}{c}{GMEAN-4.0}   & \multicolumn{1}{c}{TOTAL\_NLL-0.25} & \multicolumn{1}{c}{TOTAL\_NLL-1.0} & \multicolumn{1}{c}{TOTAL\_NLL-4.0} \\ \midrule
AE  & Central   & \exLL{}  & 0.707 $\pm{}$ 0.001                          & 0.657                           & 0.653                           & 0.603                           & 0.615                           & 0.647                           & 0.655                               & 0.636                              & 0.65                               \\ \cmidrule(l){3-12} 
    &           & DeepLIFT                  & 0.63                           & 0.465                           & 0.437                           & 0.547                           & 0.527                           & 0.534                           & 0.588                               & 0.496                              & 0.485                              \\ \cmidrule(l){3-12} 
    &           & GradShap                  & 0.628                          & 0.494                           & 0.488                           & 0.164                           & 0.228                           & 0.248                           & 0.396                               & 0.361                              & 0.368                              \\ \cmidrule(l){2-12} 
    & Coalition & \exLL{}  & \textbackslash{}textbf\{0.72\} & \textbackslash{}textbf\{0.699\} & \textbackslash{}textbf\{0.698\} & 0.607                           & 0.605                           & 0.596                           & 0.664                               & 0.652                              & 0.647                              \\ \midrule
BAE & Central   & \exLL{}  & 0.702                          & 0.644                           & 0.641                           & 0.628                           & 0.642                           & 0.63                         & 0.665                               & 0.643                              & 0.635                              \\ \cmidrule(l){3-12} 
    &           & \textbackslash{}varLL\{\} & 0.62                           & 0.548                           & 0.578                           & \textbf{0.848} & \textbackslash{}textbf\{0.924\} & \textbf\{0.936\} & \textbf{0.734}     & \textbackslash{}textbf\{0.736\}    & \textbf{0.757}    \\ \cmidrule(l){2-12} 
    & Coalition & \exLL{}  & \textbackslash{}textbf\{0.72\} & 0.693                           & \textbackslash{}textbf\{0.698\} & 0.602                           & 0.606                           & 0.619                           & 0.661                               & 0.65                               & 0.658                              \\ \cmidrule(l){3-12} 
    &           & \textbackslash{}varLL\{\} & 0.713                          & \textbackslash{}textbf\{0.752\} & \textbackslash{}textbf\{0.722\} & \textbackslash{}textbf\{0.803\} & \textbackslash{}textbf\{0.895\} & \textbackslash{}textbf\{0.832\} & \textbackslash{}textbf\{0.758\}     & \textbackslash{}textbf\{0.824\}    & \textbackslash{}textbf\{0.777\}    \\ \bottomrule
\end{tabular}
\end{table}
